Constraint Satisfaction Problems with Advice

We initiate the study of algorithms for constraint satisfaction problems with ML oracle advice. We introduce two models of advice and then design approximation algorithms for Max Cut, Max $2$-Lin, and Max $3$-Lin in these models. In particular, we show the following. 1. For Max-Cut and Max $2$-Lin, we design an algorithm that yields near-optimal solutions when the average degree is larger than a threshold degree, which only depends on the amount of advice and is independent of the instance size. We also give an algorithm for nearly satisfiable Max $3$-Lin instances with quantitatively similar guarantees. 2. Further, we provide impossibility results for algorithms in these models. In particular, under standard complexity assumptions, we show that Max $3$-Lin is still $1/2 + \eta$ hard to approximate given access to advice, when there are no assumptions on the instance degree distribution. Additionally, we also show that Max $4$-Lin is $1/2 + \eta$ hard to approximate even when the average degree of the instance is linear in the number of variables.

==> hardness.tex <==
\section{Deterministic Simulation of Advice}

We recall the following lemma that relates the probability of an event under two distributions as a function of their KL divergence.

\begin{lemma}			\label{lem:kl-div}
	Consider two probability distributions $P,Q$ over the same sample space $\Omega$. Then for any event $\cE \subset \Omega$, we have
	\[
	Q(\cE) \leq \max\left(\frac{2 d_{\rm KL}(Q,P)}{-\log P(\cE) + 1}, e\sqrt{2P(\cE)}\right).
	\] 	
\end{lemma}

Now, given a string $x^* \in \{\pm 1\}^n$, let $y$ be an $\epsilon$-correlated copy of $x$, and let $Q$ denote the distribution corresponding to $y$. Furthermore, let $P$ denote the uniform distribution over $\{\pm 1\}^n$. For $i \in [n]$, let $P_i$ and $Q_i$ denote the distribution corresponding to the $i^{th}$ coordinate.

\begin{claim}			\label{cl:kl-div}
	\[
	d_{\rm KL}(Q,P) \leq 4\epsilon.
	\]
\end{claim}
\begin{proof}
	Using the chain rule for KL divergence, we get that 
	\[
	d_{\rm KL}(Q,P) = \sum_{i \in [n]} d_{\rm KL}(Q_i,P_i) = n \left(\left(\frac12 + \epsilon\right)\log\frac{1/2 + \epsilon}{1/2} + \left(\frac12 - \epsilon\right)\log\frac{1/2 - \epsilon}{1/2}\right) \leq 4\epsilon. 
	\]
\end{proof}

Let $\cE \subseteq \{\pm 1\}^n$ denote the set of oracle advice under which the algorithm succeeds in recovering a $(1 - \eta)$-approximate solution. The following lemma lower bounds the mass of $\cE$ under the uniform distribution.

\begin{lemma}				\label{lem:kl-lower}
	\[
	P(\cE) \geq 2^{-10\epsilon n}.
	\]
\end{lemma}
\begin{proof}
	Recall that from Lemma \ref{lem:kl-div}, we have that
	\[
	1 - \eta \leq Q(\cE) \leq \max\left(\frac{2 d_{\rm KL}(Q,P)}{-\log P(\cE) + 1}, e\sqrt{2P(\cE)}\right)
	\leq \max\left(\frac{8\epsilon n}{-\log P(\cE) + 1}, e\sqrt{2P(\cE)}\right)
	\]
	Without loss of generality, we may 
	\[
	\frac{8 \epsilon n}{-\log P(\cE) + 1} \geq e\sqrt{P(\cE)},
	\]	
	otherwise, we have that $P(\cE) \geq \Omega(1)$, which would imply the claim. Therefore,
	\[
	\frac{8\epsilon n}{-\log(P(\cE)) + 1} \geq 1 - \eta,
	\]
	which on rearranging implies that
	\[
	\log\frac{1}{P(\cE)} \leq 10\epsilon n,
	\]
	or, $P(\cE) \geq 2^{-10\epsilon n}$.
\end{proof}

The above lemma immediately implies the following corollary.

\begin{corollary}					\label{corr:kl-bound}
	The following holds for any $\epsilon < \epsilon_0$. Let $\cI$ be a family of CSP instances with the following property. Suppose there exists an algorithm, that on input instance $I \in \cI$, with an access to $\epsilon$-correlation oracle, outputs a $(1 - \eta)$-approximate solution to $I$ in time ${\rm poly}(|I|)$ with $\Omega(1)$ probability over the oracle's advice. Then there exists a randomized polynomial time algorithm that runs in time $2^{10\epsilon|I|}$ and produces an $1 - \eta$-approximate solution to $P$, for every $P \in P$.
\end{corollary}
\begin{proof}
	Fix the instance size $n$, and let $I \in \cI$ be a CSP $n$ vertices. Let $Q$ denote the distribution over the oracle advice, and let $\cE \subseteq \{\pm \}^n$ be the set of advice on which the algorithm outputs a $(1 - \eta)$-approximate solution. Since the setting implies that $Q(\cE) \geq \Omega(1)$, denoting $P$ as the uniform distribution over $\{\pm 1\}^n$, using Lemma \ref{lem:kl-lower} we have that
	\[
	P(\cE) \geq 2^{-10\epsilon n}
	\]
	Therefore, among $N:= 2^{10\epsilon}\log(1/\delta)$-uniformly random draws of strings from $\{\pm 1\}^n$, with probability at least $1 - \delta$, at least one of the strings belongs to $\cE$. Hence, trying out the algorithm with all $N$-draws as the oracle advice, at least one of the trials of the algorithm will output a $1 - \eta$-approximate solution.
\end{proof}

{\bf Connection to SETH}. We will call a family of $\cP$ as $\epsilon_0$-advice solvable, if it satisfies the premise of Corollary \ref{corr:kl-bound} with $\epsilon = \epsilon_0$. The following is an immediate consequence of the above:

\begin{lemma}
	Let $\cP$ be a family of problems for which there is no $2^{\epsilon n}$ time $(1 - \eta)$-approximation algorithm. Then, $\cP$ cannot be approximated upto factor $1 - \eta$ by algorithms with access to $\epsilon/100$-correlated oracle advice.
\end{lemma}

{\bf Near Sub-exponential Time Algorithms}. {\bf TBD}





 


	
	
			

==> max-cut.tex <==
\section{Max Cut}

We give a $(1 - o(1))$-approximation algorithm for Max-Cut in the presence of label advice. The description of the algorithm is given in the figure below.

\begin{figure}[ht!]
	\begin{mdframed}
		{\bf Input}: A $d$-regular graph $G = (V,E)$ and $\{\pm 1\}$-valued label advice $\{x_i\}_{i \in V}$ generated with respect to an optimal partition $(S^*,T^*)$; here $x_i=1$ and $x_i = -1$ indicate membership in $S^*$ and $T^*$ respectively.\\[2pt]
		{\bf Algorithm}:
		\begin{enumerate}
			\item For every vertex $i \in V$, define $\Delta_i$ as 
			\[
			\Delta_i = \sum_{j \in N_G(i)} x_j.
			\]
			\item Define $V_L$ as the set of vertices
			\[
			V_L := \left\{i \in V~\Big|~|\Delta_i| \geq 20\sqrt{d\log n} \right\}.
			\]
			\item Define the sets $S_L := \{i \in V_L \Big| \Delta_i \leq 0 \}$, $T_L := V_L \setminus S_L$ and $Q:= V \setminus V_L$. 
			\item For every $i \in Q$, define $d_S(i) := |E(i,S_L)|$ and $d_T(i) := |E(i,T_L)|$.
			\item Solve the following linear program:
			\begin{eqnarray}
				\textnormal{Maximize} & \sum_{i \in Q} \left(\theta_id_T(i) + (1 - \theta_i)d_S(i)\right)  & \\
				\textnormal{Subject to} & d_T(i) + \sum_{j \in N_G(i) \cap Q}~(1-\theta_j) \in [d/2 \pm \delta]  & \forall i \in Q,
				\label{eqn:cons-1}\\
				& d_S(i) + \sum_{j \in N_G(i) \cap Q}~\theta_j \in [d/2 \pm \delta]  & \forall i \in Q,
				\label{eqn:cons-2}\\
				& \theta_i \in [0,1] & \forall i \in Q,
				\label{eqn:cons-3}
			\end{eqnarray}
			where $\delta := 30\sqrt{d\log n}/\epsilon$. 
			\label{step:lp} 
			\item Sample $y_i \sim \{0,1\}_{\theta_i}$ for every $i \in Q$ independently.
			\item Output partition $(S,T)$ where
			\[
			S:= S_L \cup \left\{i \in Q \Big| y_i = 1 \right\}
			\ \ \ \ \ \ \textnormal{and} \ \ \ \ \ \ \
			T:= T_L \cup \left\{i \in Q \Big| y_i = 0 \right\}.
			\]
		\end{enumerate}
	\end{mdframed}
	\caption{Max-Cut with Label Advice}
	\label{fig:max-cut}
\end{figure}

The following lemma summarizes the guarantees of the above algorithm.

\begin{theorem}				\label{lem:alg}
Suppose $G = (V,E)$ is a $d$-regular graph with $d \geq \log^3 n$. Furthermore, let $\{x_i\}_{i \in V}$ be an $\epsilon$-correlated label advice generated with respect to a fixed optimal cut in $G$. Then the algorithm in Figure \ref{fig:max-cut} outputs a cut of value at least $(1 - o(1)){\sf Opt}(G)$ with probability at least $1 - 1/n$ over the generation of the label advice $x$. 
\end{theorem}

In the following sections we analyze the algorithm and establish the above lemma.


\section{Analysis of Algorithm \ref{fig:max-cut}}

Before we analyze the algorithm, let us introduce some notation. Let $(S^*,T^*)$ denote the optimal partition from which the label advice $\{x_i\}_{i \in V}$ is generated. For a pair of disjoint subsets $A,B \subseteq V$ we will use $E[A,B]$ to denote the set of edges going from $A$ to $B$. For a vertex $i$ and a set $A \not\ni i$, we use $E(i,A)$ to denote the set of edges from $i$ to $A$.

\subsection{Properties of $S_L,T_L$, and $Q$}

In this section, we establish some properties of the sets $S_L,T_L$, and $Q$, which will hold with high probability over the generation of the label advice $\{x_i\}_{i \in V}$. We start with the following basic observation.

\begin{observation}				\label{obs:ob-1}
	Randomizing over the label advice, for every $i \in V$, we have that 
	\[
	\Ex\left[\Delta_i\right] = 2\epsilon \Delta^*_i,
	\]
	where $\Delta^*_i := |E(i,S^*)| - |E(i,T^*)|$.
\end{observation}

Next, we have the following claim which gives a tail bound for $\Delta_i$.

\begin{claim}			\label{cl:cl-1}
	Randomizing over the generation of the label advice $\{x_i\}_{i \in V}$, we have that 
	\begin{equation}				\label{eqn:conc}
		\Pr_x\left[\forall~i \in V, \Big|\Delta_i - \Ex\left[\Delta_i\right]\Big| \leq 4\sqrt{d \log n}\right] \geq 1 - 1/(2n).
	\end{equation}
\end{claim}
\begin{proof}
	For any $i \in V$, note that $\Delta_i = \sum_{j \in N_G(i)} x_j$ is a sum of $d$ independent $\{\pm 1\}$-valued random variables. Therefore, using Hoeffding's inequality we get that:
	\[
	\Pr_x\left[\left|\Delta_i - \Ex\left[\Delta_i\right]\right| \geq 4\sqrt{d \log n}\right] \leq 2\exp\left(-\frac{16 d \log n}{8d}\right) = 2n^{-2}.
	\]
	The claim now follows by taking a union bound over all $i \in V$.
\end{proof}

Using the above, we derive a couple of lemmas that establish some useful properties that will be used frequently in the analysis.

\begin{lemma}					\label{lem:cond-1}
	Assuming that the event from Claim \ref{cl:cl-1} holds, we have $S_L \subseteq S^*$ and $T_L \subseteq T^*$.
\end{lemma}
\begin{proof}
	We will prove that $S_L \subseteq S^*$, the argument for $T_L \subseteq T^*$ is identical. Fix a vertex $i \in S_L$. Since \eqref{eqn:conc} holds in the setting of the lemma, using Observation \ref{obs:ob-1} we have that
	\[
	\Delta^*_i = \frac{\Ex\left[\Delta_i\right]}{2\epsilon} \leq \frac{\Delta_i + 10\sqrt{d \log n}}{2\epsilon} \leq \frac{-10\sqrt{d \log n}}{2\epsilon} < 0,
	\]
	i.e., in other words $|E(i,S^*)| \leq |E(i,T^*)|$. But then $(S^*,T^*)$ is an optimal partition, and hence we must have that $i \in S^*$ (since putting $i \in T^*$ will not increase the value of the cut). Since the above argument holds for any $i \in S_L$, we have that $S_L \subseteq S^*$.  
\end{proof}

\begin{lemma}					\label{lem:cond-2}
	Assuming that the event from Claim \ref{cl:cl-1} holds, for every $i \in Q$ we have
	\[
	|\Delta^*_i| \leq \frac{30\sqrt{d \log n }}{\epsilon}.
	\]
\end{lemma}
\begin{proof}
	Fix an vertex $i \in Q$. Then,
	\begin{equation}
		\Delta^*_i 
		= \frac{\Ex\left[\Delta_i\right]}{2\epsilon}				
		\leq \frac{\Delta_i + 10\sqrt{d\log n}}{2\epsilon} 		
		\leq \frac{15\sqrt{d \log n}}{\epsilon},			\label{eqn:bd-1}
	\end{equation}		
	where the last step uses the observation that since $i \in Q$, we have $\Delta_i \leq 20\sqrt{d\log n}$. An identical argument also gives the bound
	\begin{equation}					\label{eqn:bd-2}
		\Delta^*_i \geq -\frac{15\sqrt{d\log n}}{\epsilon}.
	\end{equation}
	Combining \eqref{eqn:bd-1} and \eqref{eqn:bd-2} gives us the bound stated in the lemma.
\end{proof}


\section{Analyzing the LP}

Next we analyze the guarantees of the LP and the rounding step. Throughout this section, we will assume that the events from Lemmas \ref{lem:cond-1} and \ref{lem:cond-2} hold. Our first lemma establishes the feasibility and bounds the optimal value of the LP.

\begin{lemma}				\label{lem:lp}
	Assume that the events from Lemma \ref{lem:cond-1} and \ref{lem:cond-2} hold. Then the LP from Figure \ref{fig:max-cut} is feasible, and its value is at least $|E[Q \cap S^*,T_L]| + |E[Q \cap T^*,S_L]|$.
\end{lemma}
\begin{proof}
	Consider the assignment $\{\theta_i\}_{i \in Q}$ where for every $i \in Q$, assign $\theta_i := \mathbbm{1}(i \in S^*)$. We claim that this is a feasible assignment to the LP. To begin with, for the first constraint, observe that for any $i \in Q$, we have
	\begin{align*}
		d_T(i) + \sum_{j \in N_G(i) \cap Q} \left(1- \theta_j\right) 
		= \Big|E(i,T_L)\Big| + \Big|E(i, T^* \setminus T_L)\Big|		
		&= \Big|E(i,T^*)\Big|		\\
		& \in \left[\frac{d}{2} \pm \Delta^*_i\right] 			\tag{Using Definition of $\Delta^*_i$}\\
		&\subseteq \left[\frac{d}{2} \pm \frac{30\sqrt{d\log n}}{\epsilon}\right] 			\tag{Using Lemma \ref{lem:cond-2}}\\ 
		&= \left[\frac{d}{2} \pm \delta\right], 				\tag{Using choice of $\delta$}								
	\end{align*} 
	i.e., this establishes that assignment satisfies \eqref{eqn:cons-1}. An identical computation also shows that for any $i \in Q$, the assignment satisfies 
	\[
	d_S(i) + \sum_{j \in N_G(i) \cap Q} \theta_j \in \left[\frac{d}{2} \pm \delta\right], 
	\]
	the assignment satisfies \eqref{eqn:cons-2} as well. Finally, since the assignment is $\{0,1\}$-valued, it satisfies \eqref{eqn:cons-3} trivially. In summary, we can conclude that the assignment $\{\theta_i\}_{i \in V}$ satisfies all the constraints, and hence the linear program is feasible.
	
	Since the above assignment is feasible, we can lower bound the value of the LP as 
	\[
	{\sf LP} \geq \sum_{i \in Q} \theta_id_T(i) + \sum_{i \in Q}(1 - \theta_i)d_S(i) = \sum_{i \in Q \cap S^*}d_T(i) + \sum_{i \in Q \cap T^*} d_S(i)
	= |E[Q \cap S^*,T_L]| + |E[Q \cap T^*,S_L]|,
	\]
	which concludes the proof of the lemma.
\end{proof}

\subsection{Rounding Step Analysis}

Let $\{\theta\}_{i \in Q}$ denote the optimal solution of the linear program. Our first lemma shows that with high probability, the neighborhood of vertices in $Q$ are {\em nearly balanced} w.r.t the partition $(S,T)$.

\begin{lemma}						\label{lem:round-1}
	With probability at least $1 - 1/n$ over $(S,T)$, we have that for every $i \in Q$, 
	\[
	\max\{|E(i,S)|,|E(i,T)|\} \leq \frac{d}{2} + 2\delta.
	\]
	Consequently, we also have that for every $i \in Q$,
	\[
	\min\{|E(i,S)|,|E(i,T)|\} \geq \frac{d}{2} - 2\delta.
	\]
\end{lemma}
\begin{proof}
	We begin by observing that
	\[
	|E(i,S)| = d_S(i) + \sum_{j \in N_G(i) \cap Q} y_j.
	\]
	Furthermore, since for every $j \in Q$, the variable $y_j$ is distributed as ${\sf Bern}(\theta_j)$, we have that
	\[
	\Ex\left[\sum_{j \in N_G(i) \cap Q} y_j\right] = \sum_{j \in N_G(i) \cap Q} \Ex\big[y_j\big] = \sum_{j \in N_G(i) \cap Q} \theta_j.
	\]
	Since $y_j$'s are independent $\{0,1\}$-valued random variables, using Hoeffding's inequality, we can bound
	\[
	\Pr\left[\left|\sum_{j \in N_G(i) \cap Q} y_j - \sum_{j \in N_G(i) \cap Q} \theta_j\right| \geq 4\sqrt{d\log(n)}\right]
	\leq 2\exp\left(-\frac{16d \log(n)}{2d} \right) \leq n^{-2}/2.
	\]
	Then using the above, we have that with probability at least $1 - 1/2n^2$, we have that 
	\[
	|E(i,S)| = d_S(i) + \sum_{j \in N_G(i) \cap Q} y_j \leq d_S(i) + \sum_{j \in N_G(i) \cap Q} \theta_j \leq \frac{d}{2} + \delta + 4\sqrt{d\log(n)}
	\leq \frac{d}{2} + 2\delta,
	\]
	where the second inequality follows using the first constraint of the LP. An identical argument using the second constraint of the LP will also show that with probability at least $1 - 1/2n^2$, we have $|E(i,T)| \leq d/2 + 2\delta$. The claim then follows by taking a union bound over all $i \in Q$.
\end{proof}

Next, let $F(y)$ denote the value of the objective with respect to the rounded solution i.e.,
\[
F(y) := \sum_{i \in Q} y_i d_{T}(i) + (1 - y_i)d_S(i).
\]
The following lemma gives a high-probability lower bound for $F(y)$.

\begin{lemma}						\label{lem:round-2}
	With probability at least $1 - 1/n$ we have that $|F(y) - \Ex\left[F(y)\right]| \leq 4d\sqrt{n \log n}$.
\end{lemma}
\begin{proof}
	We rearrange the expression of $F(y)$ as 
	\[
	F(y) = \sum_{i \in Q} d_S(i) + \sum_{i \in Q} y_i(d_T(i) - d_S(i))
	\]
	Note that the second summation term above (denoted as $F'(y)$) is a weighted-sum of independent $\{0,1\}$-valued random variables where the coefficient of each random variable is bounded in $[-d,d]$. Therefore, for a fixing of $\{x_i\}_{i \in V}$ and randomizing over the choice of $\{y_i\}_{i \in Q}$, using Hoeffding's inequality we get that: 
	\[
	\Pr\left[\Big|F'(y) - \Ex\left[F'(y)\right]\Big| \geq 4d\sqrt{n\log n}\right]
	\leq 2\exp\left(-\frac{16d^2n\log(n)}{8|Q|d^2}\right) \leq 1/n.
	\]
	Therefore, with probability at least $1 - 1/n$, we have that 
	\[
	\left|F(y) - \Ex\big[F(y)\big]\right| = \left|F'(y) - \Ex\big[F'(y)\big]\right| \leq 4d\sqrt{n \log(n)}.
	\]	
\end{proof}


\subsection{Bounding the Cut Value}

Now we are ready to analyze the value of the cut returned by the algorithm. Let us assume that the events from Lemmas \ref{lem:round-1} and \ref{lem:round-2} hold. Recall that $(S,T)$ is the partition returned by the algorithm. Since $S_L \subseteq S$ and $T_L \subseteq T$ by construction, we can write the value of the corresponding cut in the following form:
\begin{equation}				\label{eqn:cut-val}
	|E[S,T]| = |E[S_L,T_L]| + \Big(|E[Q \cap S, T_L] + |E[Q \cap T, S_L]|\Big) + |E[Q \cap S, Q\cap T]|.
\end{equation}
Let $d_{\rm out}(i)$ denote the number of edges incident on $i$ that are cut in the partition $(S,T)$. The following lemma rearranges the second and third term of the above into a more convenient form.
\begin{lemma}					\label{lem:cut-1}
	\[
	\Big(|E[Q \cap S, T_L] + |E[Q \cap T, S_L]|\Big) + |E[Q \cap S, Q\cap T]| = 
	\frac{F(y)}{2} + \frac12\sum_{i \in Q}d_{\rm out}(i).
	\]
\end{lemma}
\begin{proof}
	Note that by definition, we have 
	\begin{equation}		\label{eqn:eq-1}
		|E[Q \cap S, T_L] + |E[Q \cap T, S_L]| = \sum_{i \in Q} y_id_T(i) + (1 - y_i)d_S(i) = F(y).
	\end{equation}
	On the other hand, we have 
	\begin{align}
		|E[Q \cap S, Q \cap T]| 
		&= \frac12\sum_{i \in Q} \Big(d_{\rm out}(i) - \mathbbm{1}(i \in S)|E(i,T_L)| - \mathbbm{1}(i \in T)|E(i,S_L)|\Big) \\  
		&= \frac12\sum_{i \in Q} d_{\rm out}(i) - \frac12\sum_{i \in Q} \Big(\mathbbm{1}(i \in S)|E(i,T_L)| + \mathbbm{1}(i \in T)|E(i,S_L)|\Big) \\
		&= \frac12\sum_{i \in Q} d_{\rm out}(i) - \frac12\Big(|E(Q \cap S,T_L)| + |E(Q \cap T,S_L)|\Big) \\
		&= \frac12\sum_{i \in Q} d_{\rm out}(i) - F(y)/2,				\label{eqn:eq-2} 
	\end{align}
	where the last step follows using \eqref{eqn:eq-1}.
	Therefore, combining \eqref{eqn:eq-1} and \eqref{eqn:eq-2} we get that 
	\begin{align*}
		|E[Q \cap S, T_L] + |E[Q \cap T, S_L]| + |E[Q \cap S, Q\cap T]|  
		&= F(y) + \frac12\sum_{i \in Q} d_{\rm out}(i) - \frac{F(y)}{2} \\ 
		&= \frac{F(y)}{2} + \frac12\sum_{i \in Q}d_{\rm out}(i).
	\end{align*}
\end{proof}
Next, we have the following lemma which further lower bounds $F(y)$.
\begin{lemma}				\label{lem:cut-2}
	Assume that the events from Lemmas \ref{lem:round-1} and \ref{lem:round-2} hold. Then,
	\[
	F(y) \geq |E[Q \cap T^*, S_L]| + |E[Q \cap S^*,T_L]| - 4d\sqrt{n \log n}.
	\] 
\end{lemma}
\begin{proof}
	To begin with, using Lemma \ref{lem:round-2} we have that 
	\begin{equation}			\label{eqn:exp-1}
		F(y) \geq \Ex\left[F(y)\right] - 4d\sqrt{n \log n}.
	\end{equation}
	Furthermore, we can expand and lower bound the expectation term as 
	\begin{align*}
		\Ex\left[F(y)\right] 
		&= \sum_{i \in Q} \Ex\left[y_id_T(i) + (1 - y_i)d_S(i)\right] \\
		&= \sum_{i \in Q} \theta_id_T(i) + (1 - \theta_i)d_S(i) \\
		&\geq |E[Q \cap S^*, T_L]| + |E[Q \cap T^*, S_L]|,
	\end{align*}
	where the last step uses the observation that the summation term is exactly the value of the LP, and hence it can be lower bounded using Lemma \ref{lem:lp}. Plugging in the above bound into \eqref{eqn:exp-1} finishes the proof.
\end{proof}


{\bf Proof of Lemma \ref{lem:alg}}. Now we put together the bounds from the above lemmas to bound the value of the cut:
\begin{align*}
	|E[S,T]| 
	&= |E[S_L,T_L]| + \Big(|E[Q \cap S, T_L]| + |E[Q \cap T, S_L]|\Big) + |E[Q \cap S, Q\cap T]| \\
	&\overset{1}{=} |E[S_L,T_L]| + \frac{F(y)}{2} + \frac12\sum_{i \in Q}d_{\rm out}(i) \\
	&\overset{2}{\geq} |E[S_L,T_L]| + \frac12\Big(|E[Q \cap S^*, T_L]| + |E[Q \cap T^*, S_L]|\Big) + \frac12\sum_{i \in Q} d_{\rm out}(i) - 4d\sqrt{n \log n} \\
	&\overset{3}{\geq} |E[S_L,T_L]| + \frac12\Big(|E[Q \cap S^*, T_L]| + |E[Q \cap T^*, S_L]|\Big) + \frac{d|Q|}{4} - 4d\sqrt{n \log n} - 2|Q|\delta 
	\\
	&\overset{4}{\geq} |E[S_L,T_L]| + \frac12\Big(|E[Q \cap S^*, T_L]| + |E[Q \cap T^*, S_L]|\Big) + \frac12\sum_{i \in Q}d^*_{\rm out}(i) - 4d\sqrt{n \log n} - 4|Q|\delta \\
	&\overset{5}{=}|E[S_L,T_L]| + \Big(|E[Q \cap S^*, T_L]| + |E[Q \cap T^*, S_L]|\Big) + |E[S^* \cap Q, S^* \cap T]| - 4d\sqrt{n \log n} - 4|Q|\delta \\
	&\overset{6}{\geq} |E[S^*,T^*]| - 4d\sqrt{n \log n} - \frac{4\cdot30n\sqrt{d \log n}}{\epsilon} 			\\
	&\geq |E[S^*,T^*]|(1 - o_n(1)).
\end{align*}
We justify the various steps above. Steps $1$ and $2$ follow using Lemma \ref{lem:cut-1} and Lemma \ref{lem:cut-2} respectively. Step $3$ uses the fact that since Lemma \ref{lem:cond-1} holds, using Lemma \ref{lem:round-1} we can bound $d_{\rm out}(i) \geq d/2 - 2\delta$ for every $i \in Q$. Step $4$ is due to the observation that for every $i \in Q$, again we can bound $d^*_{\rm out}(i) \leq d/2 + \Delta^*_i \leq d/2 + 2\delta$. Step $5$ follows using arguments identical to Lemma \ref{lem:cut-1} applied to the partition $(S^*,T^*)$. In step $6$, we observe that since $S_L \subseteq S^*$ and $T_L \subseteq T^*$ (due to Lemma \ref{lem:cond-1}), we have that 
\[
|E[S^*,T^*]| = |E[S_L,T_L]| + \Big(|E[Q \cap S^*, T_L]| + |E[Q \cap T^*, S_L]|\Big) + |E[S^* \cap Q, S^* \cap T]|.
\]
Finally, in the last step we use the fact that the value of the optimal cut is at least $nd/2$ and $d \geq \log^3 n$ in the setting of Lemma \ref{lem:alg}.


==> misc.tex <==
\subsection{Miscellaneous}

\begin{fact}
	The following holds for any $i \in [n]$. Given $z \in [-1,1]^n$, we can efficiently find $z' \in [-1,1]$ such that 
	\[
	z'_j  
	\begin{cases}
		\in \{\pm 1\} & \mbox{ if } j = i, \\
		= z_i & \mbox{ if } j \neq i,
	\end{cases}
	\]
	and $\langle z', A z' \rangle \geq \langle z, A z \rangle$.
\end{fact}
\begin{proof}
 	Given $\theta \in [-1,1]$, let $z'(\theta)$ be the vector 
 	\[
 	z'(\theta)_i = 
 	\begin{cases}
 		\theta & \mbox{ if } j = i, \\
 		z_j & \mbox{ otherwise.}
 	\end{cases}
 	\]
	Since the diagonal entries of $A$ are $0$ note that the map $\theta \to \langle z'(\theta), A z'(\theta) \rangle$ is linear in $\theta$ and hence its maximum value within the interval $[-1,1]$ is attained at one of the end-points $\theta^* \in \{\pm 1\}$; hence $z' = z'(\theta^*)$ satisfies the guarantee of the claim. 
\end{proof}
